Entanglement spectra from holography

The entanglement spectrum of a bipartite quantum system is given by the distribution of eigenvalues of the modular Hamiltonian. In this work, we compute the entanglement spectrum in the vacuum state for a subregion of a $d$-dimensional conformal field theory (CFT) admitting a holographic dual. In the case of a spherical (or planar) entangling surface, we recover known results in two dimensions, including the Cardy formula in the high energy regime. In higher dimensions $d>2$, we analytically determine a generalization of the Cardy formula valid at large energies and consistent with previous studies of CFT spectra in the literature. We also investigate numerically the spectrum at energy levels far above the modular ground state energy. We extend our analysis to the supersymmetric point of Einstein-Maxwell gravity, providing exact results when $d=2,3$, and a generalization of the Cardy formula at high energies in generic dimension $d$. We consider small shape deformations of a spherical entangling surface, for both the non-supersymmetric and the supersymmetric cases. In all cases we find that the high-energy scaling of the microcanonical entropy with the modular energy is unaffected by the shape deformation. This result suggests that the high-energy regime of the entanglement spectra carries universal information, independent of the shape of the entangling surface.

==> Draft_Sections/App_Gauss_Bonnet.tex <==
\section{Density of states in Gauss-Bonnet gravity}
\label{app:DOS_GB}

\SB{Since the location of branch cuts is a non-trivial problem (to which we only have numerical access), I suggest to leave it for future studies.}

\subsection{Gauss-Bonnet gravity}

In this appendix, we investigate the density of states for holographic CFTs dual to Gauss-Bonnet (GB) gravity \cite{Lovelock:1970zsf,Lovelock:1971yv,Cai:2001dz}.
The corresponding gravitational action in $d+1$ dimensions (with $d\geq 4$) reads
\begin{subequations}
\be
I_{\rm GB} = \frac{1}{2 \ell_{P}^{d-1}} \int d^{d+1} x \, \sqrt{-g} \, \left[ \mathcal{R} + \frac{d(d-1)}{\tilde{L}^2} + \frac{\lambda \tilde{L}^2}{(d-2)(d-3)} \mathcal{X}_4 \right] \, ,
\ee
\be
\mathcal{X}_4 = \mathcal{R}_{\mu\nu\rho\sigma} \mathcal{R}^{\mu\nu\rho\sigma} 
- 4 \mathcal{R}_{\mu\nu} \mathcal{R}^{\mu\nu} + \mathcal{R}^2 \, ,
\ee
\end{subequations}
where $\mathcal{X}_4$ is the four-dimensional Euler density.
Besides the Planck length $\ell_P$, this theory admits two other parameters: the coupling constant $\lambda$ of the Euler density, and the curvature scale $\tilde{L}^2=f_{\infty} \, L^2$, where $L$ is the AdS radius.
However, only one of the additional parameters is independent, since they are related by the identity
\be
1- f_{\infty} + \lambda f_{\infty}^2 = 0 \, .
\label{eq:app:relation_lambda_f}
\ee
The case of pure Einstein gravity is recovered when $\lambda=0$, or analogously $f_{\infty}=1$.
This leads us to the following guiding principle: \textit{whenever there exist multiple solutions to the equations of GB gravity, we only keep the root which reduces to Einstein gravity when $\lambda=0$.}

The above-mentioned parameters are related to the CFT data via 
\begin{subequations}
\be
\le \frac{L}{\ell_P} \ri^{d-1} = 
\frac{\Gamma(d/2)}{2 \pi^{d/2}} \, a^*_d \left[ (d-1) \frac{\tilde{C}_T}{a_d^*} - (d-3) \right] \, ,
\ee
\be
\lambda f_{\infty} = \frac{d-3}{2} \, 
\frac{\le \tilde{C}_T/a_d^* \ri -1}{(d-1) \le \tilde{C}_T/a_d^* \ri - (d-3)} \, ,
\ee
\label{eq:holo_dictionary_GB}
\end{subequations}
where $\tilde{C}_T$ is proportional to the central charge \eqref{eq:def_CT} entering the two-point function of the energy-momentum tensor, and  $a^*_d$ is the central charge appearing in front of the type-A anomaly \cite{Deser:1993yx}.
They are normalized such that $\tilde{C}_T|_{d=4}= c$ and $a^*_4 = a$, where $a,c$ are the central charges entering the four-dimensional Weyl anomaly \cite{Komargodski:2011vj}. 

On the CFT side, one can perform the same mapping to hyperbolic space explained in section \ref{eq:CHM_hyperbolic_space}, and then look for a black hole solution of GB gravity with boundary $S^1 \times H^{d-1}$.
It turns out that the metric takes the same spherically-symmetric form in eq.~\eqref{eq:metric_BH}, but now the blackening factor is given by
\be
G(r) = \frac{r^2}{2 \lambda L^2} \left[ 1- \sqrt{1-4 \lambda \le 1- \frac{m}{r^d} \ri} \right] -1 \, ,
\ee
where $m$ is a mass parameter, related to the energy density of the black hole.
In particular, one can define the quantity $f_{\infty}$ in terms of the asymptotic value of the blackening factor at the boundary, \ie 
\be
f_{\infty} = \lim_{r \rightarrow \infty} \le \frac{L^2}{r^2} G(r) + 1 \ri = \frac{1}{2\lambda} \le 1- \sqrt{1-4\lambda} \ri \, .
\label{eq:app:finfty}
\ee
We stress that while there exists another blackening factor satisfying the equations of motion of GB gravity, we only keep this solution because it reduces to Einstein gravity in the limit $\lambda \rightarrow 0$ \cite{Myers:2010ru}.
Moreover, one can also show that the other solution leads to ghosts and non-unitarity of the boundary theory \cite{PhysRevLett.55.2656,Myers:2010ru}.
Instead, demanding that the dual theory is causal and does not generate negative energy excitations lead to further constraints on the coupling constants \cite{Brigante:2007nu,Brigante:2008gz,Buchel:2009tt,Buchel:2009sk,Hofman:2009ug,Ge:2009eh,Cai:2008ph,Cai:2009zv,deBoer:2009pn,Camanho:2009vw}
\be
- \frac{(3d+2)(d-2)}{4(d+2)^2} \leq \lambda \leq \frac{(d-2)(d-3)(d^2-d+6)}{4(d^2-3d+6)^2} \, ,
\label{eq:app:rangelambda}
\ee
which imply
\be
\frac{2(d+2)}{3d+2} \leq f_{\infty} \leq \frac{2(d^2-3d+6)}{d^2-d+6}  \, .
\label{eq:app:rangef}
\ee
In particular we always have $f_{\infty} \geq 0$, as required to define a positive curvature radius in asymptotically AdS spacetime.
The horizon entropy of the black hole reads
\be
S_{\rm therm}= 2\pi V_{\Sigma} \le \frac{1}{\ell_P} \ri^{d-1} r_h^{d-1} 
\le  1- 2 \lambda f_{\infty} \frac{d-1}{d-3} \frac{L^2}{r_h^2} \ri \, ,
\label{eq:thermalS_GB}
\ee
where $V_{\Sigma}$ is the volume of hyperbolic space introduced in eq.~\eqref{eq:def_VSigma}.

Next, one can perform the replica trick following the steps described in section~\ref{ssec:replica_trick}, and compute the holographic R\'{e}nyi entropies.
The result reads \cite{Hung:2011nu}
\be
\begin{aligned}
S_n  = \pi V_{\Sigma} \le \frac{L}{\ell_P} \ri^{d-1} \frac{n}{n-1} & \left[ \frac{1}{f_{\infty}} \le 1- x_n^d \ri - \frac{3}{d-3} \le 1- x_n^{d-2} \ri - \frac{d-1}{d-3} \, \lambda f_{\infty} \le 1- x_n^{d-4} \ri  \right. \\
& \left.  + \frac{d}{d-3} \le 1- 4 \lambda \ri \le \frac{1}{1-2 \lambda f_{\infty}}  - \frac{x_n^d}{x_n^2 -2 \lambda f_{\infty}} \ri \right] \, ,
\end{aligned}
\label{eq:Renyi_GB}
\ee
where the dimensionless horizon radius $x_n= r_h/L$ is implicitly defined by the identity 
\be
\frac{d}{f_{\infty}} x_n^4 - \frac{2}{n} x_n^3 - (d-2) x_n^2 
+ \frac{4 \lambda f_{\infty}}{n} x_n + (d-4) \lambda f_{\infty} = 0 \, .
\label{eq:def_xn_GB}
\ee
From this expression, we can compute some relevant limits.
First, one can check that $x_1 =1$ is a solution
% \ts{(if $f_\infty =(0,1)$ it looks like this is the only positive real solution, but not if $f_\infty>1$)} 
for any choice of the parameters in the range \eqref{eq:app:rangelambda}--\eqref{eq:app:rangef}.
The second interesting limit is $n \to \infty$, which admits in principle four possible solutions. 
However, the only one that reduces to the value obtained in eq.~\eqref{eq:range_xn} for Einstein gravity in the limit $\lambda \rightarrow 0$ is given by
\be
x_{\infty}^2 = \frac{1}{2d}\left[(d-2)f_\infty + \sqrt{(d^2-4d)(f_\infty-2)^2+4 f_\infty^2}\right] \, .
\ee
Finally, we consider the limit $n \rightarrow 0$, where we can find analytic solutions for $x_0$ by either assuming that this quantity is finite or divergent.
The latter case is the only one leading to the case of Einstein gravity when $\lambda \rightarrow 0$, therefore we only retain such solution. 
At leading order in $1/n$, it reads
\be
x_{n \rightarrow 0} \approx \frac{2 f_{\infty}}{d} \frac{1}{n} \, .
\label{eq:app:leading_x0}
\ee
As a consistency check, we numerically observe that demanding that the R\'{e}nyi entropies with values $n=0, \infty$ are real and positive, and that $S_{\infty} \leq S_0$, lead to the above-mentioned solutions for $x_n$.
% \be
% \begin{aligned}
% & x_\infty^2 = \frac{1}{2d}\left[(d-2)f_\infty \pm \sqrt{(d^2-4d)(f_\infty-2)^2+4 f_\infty^2}\right] \, , \\
% & \text{or} \quad  x_{\infty}^2 = \frac{1}{2d}\left[(d-2)f_\infty \pm i \sqrt{(d^2-4d)(f_\infty-2)^2+4 f_\infty^2}\right] \, .
% \end{aligned}
% \ee
% \ts{Numerically, it looks like $0<f<1$ if we demand that the renyies at $n=0$ and $n=\infty$ are positive real, and that $S_\infty \leq S_0$. In that case, also the $x_{n\to 0} = \infty$ is the consistent solution and $x_\infty^2$ with the plus sign and no $i$}
% \ts{the $n \to 0$ limit:}
% When $n \to 0$, we can find analytic solutions for $x_n$, where we either assume that $x_0$ is finite, or that it is diverging. Assuming $f\neq 1$, the finite solutions can be obtained by a expanding $x_n$ to first order in $n$,
% \be
% x^{finite}_{n\to 0} = \left((1-\frac{d}{4})n, \pm \sqrt{2-\frac{2}{f_\infty}}-\frac{d(f_\infty-2)^2}{8 f_\infty^2}n \right)
% \ee



\subsection{Computation of the density of states}

\SB{Branch points: see "Branch points" in "Holographic-DOS-Stefano.nb" under "Gauss-Bonnet gravity".}

We apply the machinery developed in section~\ref{ssec:DOS_from_Renyi} to compute the DOS using the saddle point approximation.
In order to define the integration contour for the inverse Laplace transform \eqref{invLap}, we discuss the structure of singularities of $e^{(1-n)S_n}$.
Obviously, the singularities can only arise when $(1-n)S_n$ is divergent, in correspondence with branch cuts.

Let us begin with the first class of singularities.
By inspection of the formula \eqref{eq:Renyi_GB}, a trivial essential singularity is located at $n=-\infty$.
Another possibility is that $x_n^2 = 2 \lambda f_{\infty}$, but plugging this solution inside eq.~\eqref{eq:def_xn_GB} forces the coupling constant to be $\lambda =0, \frac{1}{4}$ (equivalently, $f_{\infty}= 1,2$).
Since we do not allow restrictions on the couplings, we exclude this case.
Finally, essential singularities of the integrand can come from values of the replica index that make $x_n$ divergent.
By studying the defining identity \eqref{eq:def_xn_GB} and looking at the solution in eq.~\eqref{eq:app:leading_x0}, we conclude that there is an essential singularity at $n=0$.

\SB{Important point to discuss:}
Let us now consider the case of branch cuts for the function $x_n$ as a function of $n$.
To identify them, we notice that the identity~\eqref{eq:def_xn_GB} defines a Riemann surface, since it can be rewritten as a polynomial equation in two variables, of the form\footnote{In addition, this equation contains two independent parameter $d, \lambda$, since $f_{\infty}$ can be eliminated by using~\eqref{eq:app:finfty}.}\CN{Is it polynomial in $n$? $n$ and $x_n$ are not independent. Does that matter? Usually functions of two variables introduce a constraint between two independent variables in order to single out a surface.}
\SB{Now I have rewritten the previous sentence and added an equation. The vanishing locus of any complex polynomial in two variables defines a Riemann surface (these are called algebraic curves). Here the idea is indeed to have two variables $(n, x_n)$ that are related by the requirement $\mathcal{P}(n,x_n)=0$.}
\be
\mathcal{P}(n, x_n)=0 \, , \qquad
\mathcal{P}(n, x_n) := \frac{d}{f_{\infty}} n x_n^4 - 2 x_n^3 - (d-2) n x_n^2 
+ 4 \lambda f_{\infty} x_n + (d-4) n \lambda f_{\infty}  \, .
\ee
Branch points of a Riemann surface are characterized by the requirement that the polynomial $\mathcal{P}(n, x_n)$ has multiple roots (\eg see pag.~556 of \cite{trott2007mathematica}).
It is hard to find the general classification of branch points for the surface described by eq.~\eqref{eq:def_xn_GB} in arbitrary dimensions and for any coupling $\lambda$ in the range \eqref{eq:app:rangelambda}. 
However, the important point is that we numerically checked that we can always deform the contour $\mathcal{C}$ of the inverse Laplace transform~\eqref{invLap} such that it passes through the dominant saddle point that we will determine in eq.~\eqref{eq:saddles_GB} below.\footnote{Indeed, it is always possible to find a region connecting the original contour $\mathcal{C}$ with the dominant saddle inside which the function $e^{(1-n)S_n}$ is analytic.}

While the general computation of the DOS is challenging, we can solve the problem in the high energy limit.
This regime is defined by the condition \eqref{eq:assumptions_cutoff}.
While in GB gravity the explicit expression for the minimal eigenenergy  is cumbersome, for our purposes it is sufficient to know that 
\be
\frac{E_0}{\srigb} = \frac{1}{\srigb} \lim_{n \rightarrow \infty} S_{n} \sim \mathcal{O}(1) \, ,
\ee
where $\srigb$ is defined by using $r_h=L x_n$ inside eq.~\eqref{eq:thermalS_GB} and setting $n=1$, \ie 
\be
\srigb \equiv 2\pi V_{\Sigma} \le \frac{1}{\ell_P} \ri^{d-1} r_h^{d-1} 
\le  1- 2 \lambda f_{\infty} \frac{d-1}{d-3} \frac{L^2}{r_h^2} \ri \, .
\ee
This quantity is the GB analog of the entropy $\sri$ of Rindler AdS \eqref{Srindler} computed in Einstein gravity, since it is the thermal entropy \eqref{eq:thermalS_GB} of the vacuum solution to GB gravity.
In other words, in the high-energy regime we will simply ignore any finite constant, and keep the leading dependence on $E$.

In this regime, the saddle point condition $f'(n_*)=0$ can only be satisfied if $x_n \rightarrow \infty$, which in turn requires $n \rightarrow 0$.
By retaining only the leading order expressions obtained in eq.~\eqref{eq:app:leading_x0}, we find
\begin{subequations}
\be
f(n) \approx n \left[ E + \frac{\pi}{f_{\infty}} V_{\Sigma} \le \frac{L}{\ell_P} \ri^{d-1} x_n^d \right] \, ,
\label{eq:xn_fn_largeE_GB}
\ee
\be
f''(n) \approx \frac{d^2 (d-1)}{2 f_{\infty}^2}   \pi V_{\Sigma} \le \frac{L}{\ell_P} \ri^{d-1} \, x_{n}^{d+1} \, .
\label{eq:f2n_largeE_GB}
\ee
\end{subequations}
Therefore, the stationary points of the function $f$ are constrained by
\be
f'(n_*) \approx E + \frac{\pi}{f_{\infty}} V_{\Sigma} \le \frac{L}{\ell_P} \ri^{d-1} (1-d) x_n^d = 0 \, ,
\ee
whose solutions read
\be
x_{n_*}^{(k)} = e^{2 \pi i k/d} \, \left[ \frac{f_{\infty}}{\pi V_{\Sigma}}  \le \frac{\ell_P}{L} \ri^{d-1}  \frac{E}{d-1} \right]^{ \frac{1}{d}} \, .
\label{eq:saddles_GB}
\ee
As usual, the real and positive root gives a dominant contribution.
Plugging the expression with $k=0$ inside the function \eqref{eq:xn_fn_largeE_GB} and its second derivative \eqref{eq:f2n_largeE_GB}, we finally obtain
\begin{subequations}
\be
f(n_*) \approx \frac{2f_{\infty}}{d-1} \frac{E}{x_{n_*}} \approx 
2 \left[ \pi V_{\Sigma} \le \frac{L}{\ell_P} \frac{f_{\infty}}{d-1} \, E \ri^{d-1}   \right]^{\frac{1}{d}}   \, ,
\ee    
\be
f''(n_*) \approx \frac{d^2}{2} \left[ \frac{\pi}{d-1} V_{\Sigma} \le \frac{L}{\ell_P} \ri^{d-1} f_{\infty}^{1-d} E^{d+1} \right]^{\frac{1}{d}} \, .
\ee
\end{subequations}
These contributions lead to the following DOS
\be
D(E) \approx \frac{1}{d \sqrt{\pi}} \left[ \frac{\pi}{d-1} V_{\Sigma} \le \frac{L}{\ell_P} \ri^{d-1} f_{\infty}^{1-d} E^{d+1} \right]^{-\frac{1}{2d}}
\, \exp \left[ 2  (\pi V_{\Sigma})^{\frac{1}{d}} \le \frac{L}{\ell_P} \frac{f_{\infty}}{d-1} \, E \ri^{\frac{d-1}{d}}   \right] \, ,
\ee
and to the leading microcanonical entropy
\be
\boxed{
S(E) \approx 2 \left[ \pi V_{\Sigma} \le \frac{L}{\ell_P} \frac{f_{\infty}}{d-1} \, E \ri^{d-1}   \right]^{\frac{1}{d}}   + \dots }
\ee
We observe that the leading contribution to the DOS and to the microcanonical entropy at high energies show the same pattern as eqs.~\eqref{eq:leading_DOS_largeE} and \eqref{CardyDeformation}, which were derived for CFTs dual to Einstein gravity.
The only difference lies in the prefactors, which now involve a dependence on the two central charges via the dictionary \eqref{eq:holo_dictionary_GB}. \sch{shape dependence is probably also easy because we have the expression in our previous paper of $C_D$ when $n\rightarrow 0$; any relation to 2309.00044 of Horacio?} 














